Label-similarity Curriculum Learning

Curriculum learning can improve neural network training by guiding the optimization to desirable optima. We propose a novel curriculum learning approach for image classification that adapts the loss function by changing the label representation. The idea is to use a probability distribution over classes as target label, where the class probabilities reflect the similarity to the true class. Gradually, this label representation is shifted towards the standard one-hot-encoding. That is, in the beginning minor mistakes are corrected less than large mistakes, resembling a teaching process in which broad concepts are explained first before subtle differences are taught. The class similarity can be based on prior knowledge. For the special case of the labels being natural words, we propose a generic way to automatically compute the similarities. The natural words are embedded into Euclidean space using a standard word embedding. The probability of each class is then a function of the cosine similarity between the vector representations of the class and the true label. The proposed label-similarity curriculum learning (LCL) approach was empirically evaluated using several popular deep learning architectures for image classification tasks applied to five datasets including ImageNet, CIFAR100, and AWA2. In all scenarios, LCL was able to improve the classification accuracy on the test data compared to standard training.

==> implementation.tex <==
We have evaluated our curriculum  learning strategy on $8$ different models. Due to infrastructure limitations, we have focused on Resnet class architectures (Resnet-$50$, Resnet-$152$, Densenet-$121$, Densenet-$161$, Resnext-$101-32\times{}4d$, Resnext-$101-64\times{}4d$ ,SeResNext-$101-32\times{}4d$) and for completeness InceptionResnetv2. Since these models require moderate computational requirements they are used in practice extensively. Resnet class architectures belong to the most prominent and popular architectures for image classfication, object detection and semantic segmentation  problems \cite{ren2015faster,dai2016r,he2017mask, chen2018deeplab}. 

For all architectures for data processing and data augmentation, we have followed the experimental protocol which is described in the corresponding original publication. All experiments are conducted by using PyTorch deep learning libray\cite{paszke2017automatic}. We conduct a large scale experimantal study, therefor we have used distributed SGD algorithm \cite{goyal2017accurate} with Horovod \cite{sergeev2018horovod} support in order to scale the experimental design. The used distributed SGD algorithm \cite{goyal2017accurate} is one of the state-of-the-art methods for large scale training. It is expected to observe slight loss of performance whenever large batch size is used (please see the results presented in \cite{goyal2017accurate}). For classical ResNet architectures and DenseNet architectures, we recover the accuracy loss. For some of the  models, we are not able recover the accuracy loss compared the published baseline. However, we improve over reproduced results by using large batch solver.



%Optimisation is performed using synchronous SGD with momentum 0.9 and a mini-batch size of 1024. The initial learning rate is set to 0.6 and decreased by a factor of 10 every 30 epochs. All models are trained for 100 epochs from scratch, using the weight initialisation strategy described in [9]. 


  

==> mgqvjdvbgzvywcqgtdzyrbkbyvpwvyqs/Introduction.tex <==
When educating humans, the teaching material is typically presented
with increasing difficulty. \emph{Curriculum learning} adopts this
principle for machine learning to guide an iterative optimization
method to a desirable optimum. In curriculum learning for neural
networks as proposed by Bengio et al.~\cite{bengio2009curriculum}, the
training examples are weighted. In the beginning of the training, more
weight is put on ``easier'' examples. The weighting is gradually
changed to  uniform weights corresponding to the canonical
objective function.



\review{Inspired by Bengio et al.~\cite{bengio2009curriculum},}
we propose \emph{label-similarity curriculum learning} (LCL) as another way
to  ``learn easier aspects of the task or easier sub-tasks, and then gradually increase the difficulty level.''
%\cite{bengio2009curriculum}.
%
If a toddler who is just learning to speak points at a car and utters
``cow'', a parent will typically react with some teaching signal.
However, a young infant is not expected 
to discriminate between a cheetah and a leopard, and mixing up the two
would only lead to a very mild correction signal -- if at all.
With increasing age, smaller errors will also be communicated.

We transfer this approach to neural network training for classification
tasks. 
%The curriculum learning is based on a label similarity matrix. Given a label similarity matrix, each row describes a probability distribution over the classes. During curriculum learning, we change the representation of the labels.  
Instead of a one-hot-encoding, the target represents a probability distribution
over all possible classes. The probability of each class depends on
the similarity between the class and the true label. That is, instead
of solely belonging to its true  class, each input can also
belong to similar classes to a lesser extent.  Gradually, this label representation is shifted towards the standard one-hot-encoding, where  targets representing different classes are orthogonal. In the beginning of training, the targets of inputs with labels \texttt{cheetah} and \texttt{leopard} should almost be the same, but always be very different from \texttt{car}. During the training process, the label representation is gradually morphed into the one-hot encoding, decreasing the entropy of the distribution encoded by the target over time.  That is, in the beginning small mistakes -- in the sense that similar classes are mixed up -- are corrected less than big mistakes, resembling a teaching process in which broad concepts are
explained first before subtle differences are taught.


The question arises how to define a proper similarity between classes. One can get a label-similarity matrix based on prior knowledge or some known structure.  For the case where the similarity is not explicitly given and the labels correspond to natural language words, we propose a way to automatically infer a representation that reflects semantic similarity. We map the labels into a Euclidean space using a word embedding. Concretely, this is done  by applying a generic document embedding to a  document explaining the label (its Wikipedia entry). Then the cosine similarities between the vector representations of the label and all possible classes are  computed. Based on these values,  a distribution over the possible classes is defined which serves as the learning target. 

%
%\textbf{The cosine similarities between the vector representations of the label and all possible classes are then computed. Based on these values,  a distribution over the possible classes is defined which serves as the learning target. While our main idea is that -- in expectation -- similar words correspond to similar inputs (e.g., images) that are rather difficult to distinguish, there can, of course,  be words with different labels that are close  in the embedding space  where the corresponding inputs are easy to tell apart. }

Our way to define the target representation
resembles the idea of \emph{hierarchical loss functions}
\cite{Silla2011,DBLP:journals/corr/abs-1709-01062}  (``We define a
metric that, inter alia, can penalize failure to distinguish between a
sheepdog and a skyscraper more than failure to distinguish between a
sheepdog and a poodle.'' \cite{DBLP:journals/corr/abs-1709-01062}).
However, there are two decisive differences. First,
we propose to gradually  shift from a ``hierarchical loss'' to
a ``flat loss''.
Second,  unlike in \cite{DBLP:journals/corr/abs-1709-01062}, our approach does not necessarily presume a given hierarchy. When dealing with natural language labels, we propose a way to automatically infer the
 similarity from a generic word embedding 
 %But to get word embeddings, we assume that the labels are natural language words and that 
under the assumption that exploiting  semantic
similarity can be helpful in guiding the learning process.
% nor does it necessarily require prior knowledge. 

For evaluating  label-similarity curriculum learning (LCL), we need data with some structure in the label space that curriculum learning can exploit. Furthermore, there should be sufficiently many classes and the task should not be easy to learn. To get label similarity based on word embeddings, we need a dataset with  natural language labels. In this study, we focus on three popular benchmark datasets, ImageNet \cite{deng2009imagenet}, CIFAR100  \cite{krizhevsky2009learning}, and Animals with Attributes (AwA)  \cite{xian2018zero}.
{To show the generality of our approach, we consider different deep learning architectures, and also different preprocessing and learning processes.}
The time schedule for increasing the ``difficulty'' of the learning
task is an obvious hyperparameter, which we carefully study \ask{and show to have little importance}.

The next section points to related literature and  Section \ref{sec:proposed_method} introduces the new \emph{label-similarity curriculum learning}.
Section~\ref{sec:experiments} describes the experiments and
Section~\ref{sec:results} the results before we conclude.


==> mgqvjdvbgzvywcqgtdzyrbkbyvpwvyqs/ProposedMethod.tex <==

We assume a discrete set of training examples $(\x_1, \class_1)
,\dots,(\x_\ell, \class_\ell)  \in \mathcal X\times \mathcal C$,
with input space  $\mathcal X$ and finite label space $\mathcal C$ with
cardinality $|\mathcal C| = C$.
Let $n: \mathcal C\to \{1,\dots,C\}$ be a bijective mapping assigning 
each label to a unique integer. This allows a straight-forward
definition of the  one-hot encoding $\vec y_i\in\mathbb R^C$
for each  training example   $(\x_i, \class_i)$. The $j$-th component of $\vec
y_i$, which
is denoted by $[\vec y_i]_j$, equals 1 if \ask{$n(\class_i)=j$} and 0 otherwise.
\begin{figure*}
	\includegraphics[width=\linewidth]{figures/comparative_method_description_final.pdf}
	\caption{A deep network (left) trained with three different encodings  on a  five-class dataset  with labels Lion, 
	Tiger, Aircraft Carrier, Alaskan Wolf and Mushroom. 
	%The left side of the figure shows an example of a deep architecture. 
	The SL (standard learning,  see Section~\ref{sec:experiments} for details) column shows the label matrix for one-hot-encoding.
	When  using LS (label smoothing, see Section~\ref{sec:experiments}),  the loss between the network output and a 
	smoothed version of the label, which does not change over time, is minimized. We propose to use a probability distribution over classes as target label, 
	where the class probabilities reflect the similarity to the true class. This is shown in the  LCL column. Unlike LS the proposed label encoding changes during training and converges 
	to the original optimization problem solved when using SL.}
	\label{fig:comparative_model_exp}
\end{figure*}

\subsection{Document embedding for defining label similarity}
\label{subsec:semantic_similarity}
%\paragraph{Document embedding for defining label similarity.}
Our learning curriculum is based on the pairwise similarities between the $C$
 classes, which are defined  based on
the semantic similarity of the class labels.
Now assume that the labels are 
natural language words, for example
$\mathcal C=\{  \dots$, \texttt{flute}, $\dots$, \texttt{strawberry}, $\dots$, \texttt{backpack},
$\dots\}$.
To quantify semantic similarity, we embed the natural language labels into Euclidean
space using a word embedding \cite{DBLP:journals/corr/abs-1301-3781}
such that similar words are nearby in the new representation.

ImageNet labels are given by WordNet identifiers representing synsets, and we redefine the labels for other datasets in a similar way. First, we convert synsest to words, for example, \texttt{n02119789} to
``fox''. Then, we find the Wikipedia article describing each word, for instance, ``Orange (fruit)'' was selected for \texttt{orange}.
Then we apply \texttt{doc2vec} \cite{le2014distributed} for mapping
the article into Euclidean space.
% We have captured topic level similarity by using articles.
We used a generic   \texttt{doc2vec}  embedding trained on the
English  Wikipedia corpus.
%This article is then mapped to an Euclidean vector using  \texttt{doc2vec} .
%This results in our vector representation via trained Doc2Vec models.
This gives us the  encoding $f_{\text{enc}}:\mathcal C\to\mathbb R^d$,
mapping each class label to the corresponding Wikipedia article and
then computing the corresponding vector representation using
\texttt{doc2vec} (with $d=100$, see below).
Now we can compute the
similarity between two classes $c_i$ and $c_j$ by the cosine
similarity
\begin{equation}\label{eq:sim}
s(c_i,c_j)=\frac{\langle f_{\text{enc}}(c_i), f_{\text{enc}}(c_j)
  \rangle}{\| f_{\text{enc}}(c_i)\|\|f_{\text{enc}}(c_j)\|} \enspace,
\end{equation}
which in our setting is  always non-negative.
The resulting label dissimilarity matrix for the ImageNet labels is visualized in Figure~\ref{fig:class_dis_matrix}. 
%\textbf{We should present label similarity matrix here instead of label dis-similarity for consistency}



\begin{figure}
\centering
	\includegraphics[width=0.5\linewidth]{figures/Class_Similarity_Low_Quality.png}
	\caption{Label dissimilarity matrix visualizing $1-s(c_i,c_j)$, $1\le
          i,j\le 1000$, for ImageNet.}
	\label{fig:class_dis_matrix}
\end{figure}



\subsection{Label encoding}%\label{ch:obj_function}

We adopt the formal definition of a curriculum
from
the seminal paper by Bengio et al.~\cite{bengio2009curriculum}.
In  \cite{bengio2009curriculum}, 
a weighting of the training data is adapted, so that in the
beginning a larger weight is put on easy examples.
To distinguish this work from our approach, we refer to 
it as \emph{example-weighting curriculum}.


Let $t\ge 0$ denote some notion of  training time (e.g., a counter of
training epochs).
In \cite{bengio2009curriculum}, there is a sequence of weights
associated with each example  $i=1,\dots,\ell$, which we denote by
$w_i^{(t)}\in [0,1]$.
These weights are normalized so that $\sum_{i=1}^{\ell}w^{(t)}_i=1$ to 
describe a proper probability distribution over the training examples.
%:
%\begin{equation}\label{eq:norm}
%w_i^{(t)} = \frac{ \tilde w_i^{(t)}}{\sum_{j=1}^\ell \tilde w_j^{(t)}}  
%\end{equation}

For the weight sequence to be a proper (example-weighting) curriculum,
Bengio et al.~\cite{bengio2009curriculum} demand that the entropy of
the weights
\begin{equation}
H(\vec w^{(t)})=-\sum_{i=1}^\ell  w_i^{(t)} \ln w_i^{(t)}
\end{equation}
is monotonically increasing with $t$ (the weights should converge
to the uniform distribution).
%and that the unnormalized weights $\tilde{w}_i^{(t)}$ are non-decreasing.

We define our \emph{label-weighting curriculum}
in a similar axiomatic way. Instead of a sequence of weights for the
training examples varying with $t$, we have a sequence of label
vectors for each training example. Let $\vv_i^{(t)}$ 
denote the $C$-dimensional label vector for training pattern $i$ at time $t$.
For the sequence to be a  {label-weighting curriculum},
the entropy of the label vector components 
\begin{equation}
\forall i=1,\dots,\ell: H(\vec \vv_i^{(t)})=-\sum_{c=1}^C  [{\vec
	\vv}_i]_c^{(t)} \ln [{\vec \vv}_i]_c^{(t)}
\end{equation}
should be monotonically 
\emph{decreasing} under the constraints that for each label vector $\vec \vv_i^{(t)}$ we
have $[{\vec \vv}]_j\geq 0$ for all $j$, $\|\vec \vv_i^{(t)}\|_1=1$, and
$\operatorname{argmax}_j [{\vec \vv}]_j^{(t)} = n(c_i)$ for all $t$.
%
The conditions imply that $\vv_i$ is always an element of the
probability simplex, the class label given in the training set
always gets the highest probability, and $\vec \vv_i^{(t)}$
converges to $\vec y_i$.


% Similar as in \cite{bengio2009curriculum},
% such a sequence can be implemented using 
% unnormalized
% vectors $\tilde{\vv}_i^{(t)}$
% for each training pattern $i$, which are mapped 
% to the corresponding ${\vv}_i^{(t)}$ analogously to 
% \eqref{eq:norm}, however, they must be non-increasing.
% For example, for 
% $0<\epsilon<1$
% the simple update
% \begin{equation}\label{eq:eps}
% [\tilde {\vec \vv}_i]_j^{(t+1)} =
% \begin{cases}
% 1 & \text{if $j= n(\class_i)$}\\
% \epsilon  [\tilde{\vec \vv}_i]_j^{(t)} & \text{otherwise}\\
% \end{cases}
% \end{equation}


%such a sequence can be implemented using 
%vectors $\vv_i^{(t)}$ for each training pattern $i$.
%, however, they must be non-increasing.
We now give an example of how to adapt the label vectors. 
Similar as in \cite{bengio2009curriculum},
we define for each training example $i$
%, consider one example \(  i \) during training.  T
the simple update rule:
\begin{equation}\label{eq:eps}
[\vec \vv_i]_j^{(t+1)} =
\begin{cases}
\frac{1}{1 + \epsilon \sum_{ k \ne n(c_i) } [\vec \vv_i]_k^{(t)} }  & \text{if $j= n(\class_i)$}\\
\frac{\epsilon  [\vec \vv_i]_j^{(t)}}{1 + \epsilon \sum_{ k \ne n(c_i) } [\vec \vv_i]_k^{(t)} }   & \text{otherwise}\\
\end{cases}
\end{equation}
The constant parameter $0<\epsilon<1$ controls how quickly the label vectors converge to the one-hot-encoded labels.
This update rule  leads to a proper {label-weighting curriculum}.
During learning, the entries for all components except $n(\class_i)$ drop with
$\mathcal O(\epsilon^t)$. 
Note that $[\vec \vv_i]_{n(c_i)}^{(t+1)} \ge [\vec \vv_i]_{n(c_i)}^{(t)}$.
%
The  vectors are initialized using the label similarity defined in \eqref{eq:sim}:
\begin{equation}
  [{\vec \vv}_i]_j^{(0)} = 
  \frac{s\big( c_i, n^{-1}(j) \big)}{\sum_{k=1}^{C} s\big( c_i, n^{-1}(k) \big) }
\end{equation}
%and then normalized to get $[\vec \vv_i]_j^{(0)}$  as in Eqn. \ref{eq:norm}.
Recall that $n^{-1}(j) $ denotes  the ``$j$-th'' natural language class label. 


%The hyperparameter $\epsilon$ controls how fast the curriculum converges to one-hot-encoded labels.







\subsection{Loss function}
Let $\mathcal{L}$ be a loss function between two probability distributions and $ f_{\theta}(x)$ be the predicted distribution for example $\vec x$ for some model parameters $ \theta$. At time step $t$ we optimize
%\begin{eqnarray}
$J^{(t)}(\theta) = \sum_{i = 1}^n \mathcal{L} (f_{\theta}(\vec{x}_i), \vec \vv_i^{(t)}) + \lambda r(\theta)$,
%\enspace,
%\end{eqnarray}
where $\lambda$ is a positive constant and $r(\theta)$ is a regularization function. In this paper, the networks are trained using the standard cross-entropy loss function with normalized targets $\vec v_i$ for the inputs $\x_i$, $i=1,\dots,\ell$. Hence, in the beginning, predicting the 
correct one-hot encoded label $\vec y_i$ causes an error signal. That is, initially it is less penalized if an object is not correctly classified with maximum confidence. Later in the training process, $\vec v_i$  converges to $\vec y_i$ and  the classifier  is then pushed to build up confidence.



==> mgqvjdvbgzvywcqgtdzyrbkbyvpwvyqs/conclusion.tex <==
We proposed a novel curriculum learning approach referred to as
label-similarity curriculum learning.
In contrast to previous methods, which change the weighting of training examples,
it is based on adapting the label representation during training.
This adaptation considers the semantic similarity of labels. It implements  the basic idea that at an early stage of learning it is less important to
distinguish between similar classes compared to separating very different classes.
%

The class similarity can be based on arbitrary \emph{a  priori} knowledge, in particular on additional information not directly encoded in the training data.
For the case where the class labels are natural language words, we 
proposed a way to  automatically define class similarity via a word embedding. We also  considered other similarity measures for  datasets where these similarity measures were available.
%In all cases, our proposed method improved the baseline}. 

We extensively evaluated the approach on five datasets. For each dataset, two to three deep learning architectures proposed in the literature were considered. We looked at simple  label smoothing and, for the two smaller datasets, also at deep mutual learning (DML) as additional baselines. In each case, we considered four different training data set sizes. Each experiment was repeated four times.
%
The empirical results strongly support our approach. \emph{Label-similarity curriculum learning 
was able to improve the average classification accuracy on the test data compared to standard training in all scenarios.} 
%
The improvements achieved by our method were more pronounced for smaller training data sets.
When considering only $10\%$ of the AWA2 training data, label-similarity curriculum learning increased 
the Resnet101 top-1 test accuracy  by  more than 22 percentage points on average compared to the standard baseline.

Our curriculum learning also outperformed simple label smoothing and DML in all but a single case.  Our method turned out to be robust with respect to the choice of the single hyperparameter controlling how quickly the learning process converges to minimizing the standard cross-entropy loss. In contrast to related approaches such as knowledge distillation and DML, the additional computational and memory requirements can be neglected. 
%Choosing a slower convergence rate gave overall better results.  While the  potential of curriculum learning has been demonstrated  in previous studies, to our knowledge, our experiments are the  first that show benefits of curriculum learning on large-scale benchmark data sets  studied in the computer vision community.

The proposed  label-similarity curriculum learning is a general approach, 
which also works for settings where the class similarity is not based on the semantic similarity of natural language words (see supplementary material).
%sections  \ref{app:awa}, \ref{app:nabirds}, and \ref{app:cub}).
%and in future work it will be interesting to see whether our results carry over to other machine learning tasks where the class similarity is not based on the semantic similarity of natural language words.



%We evaluated the approach on three datasets . The labels are mapped to Euclidean space by encoding the Wikipedia article explaining the label using a generic \texttt{doc2vec} embedding. Eight deep learning systems proposed in the literature were considered. We reimplemented them closely following the original publications and existing open-source software. We trained each system three times, which resulted in an unbiased comparison of deep learning systems for ImageNet. The curriculum learning could improve the final accuracies in all cases nearly without a cost. The method turned out to be robust with respect to the choice of the single hyperparameter controlling how quickly the learning process converges to minimizing the standard cross-entropy loss. Choosing a slower convergence rate gave overall better results.  While the  potential of curriculum learning has been demonstrated  in previous studies, to our knowledge, our experiments are the  first that show benefits of curriculum learning on a  large-scale data set that has been extensively studied by the machine learning community.

==> mgqvjdvbgzvywcqgtdzyrbkbyvpwvyqs/experiments.tex <==
We evaluated our curriculum  learning strategy by running extensive experiments on ImageNet~\cite{deng2009imagenet}, CIFAR$100$~\cite{krizhevsky2009learning}, and AWA$2$~\cite{xian2018zero} plus additional experiments on CUB-200-2011 \cite{WahCUB_200_2011} and NABirds \cite{Horn_2015_CVPR} (see supplementary material).
On CUB-200-2011 and AwA2, we evaluated our approach using both the proposed semantic similarity of the labels as well as visual similarity. On NABirds, we evaluated our approach also using similarity based on the given (biological) hierarchy, where we used simrank~\cite{jeh2002simrank} for calculating the similarity matrix.

%The ImageNet dataset contains 1.28 million training images and 50000 validation images belonging to $C=1000$ natural object categories. CIFAR$100$ contains 50000 training images and 10000 test images belonging to $C=100$ natural object categories. AWA$2$ contains in total 37322 images. 
%We have conducted a detailed and extensive experimental evaluation. 
For each dataset we considered at least two different models and two different baselines. 
Descriptive statistics of the datasets and a summary of the experimental setup are given in Table \ref{tab:data_statistics} and Table \ref{tab:all_exp}. 
%We will give details of these experiments in the following subsections.
We considered different training set sizes, where $\DR\in\{5\%,10\%,20\%,100\%\}$ refers to the fraction of training data used. The remaining training data was discarded (i.e., not used in the training process at all); the test data were always the same. 

\begin{table}[ht]
\begin{center}
\caption{$\ell_{\text{train}}$ denotes the number of training images, $\ell_{\text{test}}$ denotes the number of test images and  $C$ the number of classes in a given dataset;
%. For each data set, we conducted several experiments. Different data set sizes and cooling rate parameters were considered  
DR indicates the data set sizes (percentage of $\ell_{\text{train}}$), $\epsilon$  the cooling parameters, and \#Rep  the number of repetitions with different initializations/seeds. The column Sim.{} indicates which similarity measures were used, where l stands for the semantic similarity using the word embedding of the labels, v for a  measure based on the similarity of the images, and h for similarity based on a given label hierarchy.}
\label{tab:data_statistics}
\begin{tabular}{lrrr@{\qquad}cccc}
%         & $S_{train}$ & $S_{test}$ &$S_{classes}$  \\
& $\ell_{\text{train}}$ & $\ell_{\text{test}}$ & $C$ & \textbf{DR} & \textbf{\#Rep} & $\boldsymbol{\epsilon}$ & \textbf{Sim.}\\
\midrule
AWA2     &  29865   &  7457   &  50  & $5\%$, $10\%$, $20\%$, $100\%$ & 4     & 0.9, 0.99, 0.999 & l, v \\
CIFAR100 &   50000  &   10000  &100 & $5\%$, $10\%$, $20\%$, $100\%$ & 4     & 0.9, 0.99, 0.999 & l    \\
ImageNet &   1281167  & 50000    & 1000 & $5\%$, $10\%$, $20\%$, $100\%$ & 4     & 0.9, 0.99, 0.999 & l\\   
NABirds  &23912&24615&555&100\%&4&0.9,0.99,.999& l, h\\
CUB-200-2011  &5994&5794&201&100\%&4&0.9,0.99,.999& l, v\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

We  empirically compared  the following algorithms:
\begin{enumerate}
    \setlength\itemsep{-0.2em}
        \item Label-similarity curriculum learning (LCL): Proposed method with label update rule \eqref{eq:eps}. The time step $t$ is the epoch number. 
        \item Standard Learning (SL): This is a standard  setup  with fixed one-hot encoding.
%        , 
%            \begin{equation}\label{eq:SL}
%                [\vec \vv_i]_j^{(t)} =
%                \begin{cases}
%                1 & \text{if $j= n(\class_i)$}\\
%                0  & \text{otherwise}\\
%                \end{cases}\enspace\enspace \text{for all } t.
%            \end{equation} 
    \item Label Smoothing (LS): Label smoothing uses soft targets instead of one-hot encoding. It has been argued that LS prevents the network from becoming over-confident and improves the empirical performance of the algorithm \cite{muller2019does}. For  $ 0 \leq \alpha \leq 1 $ label smoothing uses following label vector 
            \begin{equation}\label{eq:LS}
                [\vec \vv_i]_j^{(t)} =
                \begin{cases}
                (1 - \alpha) + \frac{\alpha}{C} & \text{if $j= n(\class_i)$}\\
                 \frac{\alpha}{C}  & \text{otherwise}\\
                \end{cases}\enspace\enspace \text{for all } t.
            \end{equation} 
     We set$ \alpha = 0.1 $ for the evaluations in this study.        
    \item Deep Mutual Learning (DML):  In DML, two models, referred to as \DMLone and \DMLtwo,  solve the same classification problem collaboratively and are  optimised jointly  \cite{zhang2018deep}. It uses one hot-encoding along with cross-entropy loss as in SL but adds additional terms 
    %\begin{equation}
    $\text{KL}( \hat{\vec \vv}_{\text{DML}_1}^{(t)}\,\|\, \hat{\vec \vv}_{\text{DML}_2}^{(t)} ) + \text{KL}( \hat{\vec \vv}_{\text{DML}_2}^{(t)}\,\|\,  \hat{\vec \vv}_{\text{DML}_1}^{(t)} )$,
    %\enspace,
    %\end{equation}
    where $\text{KL}$ denotes the  Kullback–Leibler  divergence
    and $\hat{\vec \vv}_{\text{DML}_1}^{(t)} $ 
    and $ \hat{\vec \vv}_{\text{DML}_2}^{(t)} $  are the predicted label probability vectors for both models. 
    We report the classification performance of both \DMLone\ and \DMLtwo.
    \item Knowledge Distillation (KD): In KD, one model is trained first using one-hot encoded targets, and then the class probabilities produced by the first model are used as ``soft targets'' for training the
    second model \cite{hinton2015distilling}.
    \item Curriculum Net (CN): In CN, example-weighted curriculum is built by sorting examples from easy to hard  \cite{guo2018curriculumnet}. 
\end{enumerate}


\begin{table*}[ht]
\begin{center}
\caption{ \ResnextSshort denotes \ResnextS, \WRNshort denotes \WRNnoblank, and \DenseNetshort denotes \DenseNet.%, DR refers to the fraction of training data used, $\epsilon$ is the cooling parameters, and \#Rep denotes the number of repetitions with different initializations/seeds.
}
\label{tab:all_exp}
\begin{tabular}{l@{\quad}c@{\quad}c}
\textbf{Model} & \textbf{Dataset}  & \textbf{Baselines} \\% \textbf{DR} & \textbf{\#Rep} & $\boldsymbol{\epsilon}$               \\
\toprule  
\ResnetES~\cite{xie2017aggregated} & CUB-200-2011  & LS, DML, SL, KD, CN \\
\ResnetVS~\cite{xie2017aggregated} & CUB-200-2011, NABirds & LS, DML, SL, KD, CN \\
\ResnetS~\cite{he2016deep} & ImageNet, NABirds & SL, LS, KD, CN  \\%   & $5\%$, $10\%$, $20\%$, $100\%$ & 4     & 0.9, 0.99, 0.999 \\ 
\ResnextSshort~\cite{xie2017aggregated} & ImageNet & SL, LS, KD, CN   \\%   & $5\%$, $10\%$, $20\%$, $100\%$ & 4     & 0.9, 0.99, 0.999 \\
\SENet~\cite{hu2018squeeze}& ImageNet & SL, LS, KD, CN   \\%   & $5\%$, $10\%$, $20\%$, $100\%$ & 4     & 0.9, 0.99, 0.999 \\
\ResnetB~\cite{he2016deep} & AWA2     & LS, DML, SL, KD, CN \\% & $5\%$, $10\%$, $20\%$, $100\%$ & 4     & 0.9, 0.99, 0.999 \\
\inceptionresnet~\cite{szegedy2017inception}& AWA2     & LS, DML, SL, KD, CN \\% & $5\%$, $10\%$, $20\%$, $100\%$ & 4     & 0.9, 0.99, 0.999 \\
\WRNshort~\cite{zagoruyko2016wide} & CIFAR100 & LS, DML, SL, KD, CN \\% & $5\%$, $10\%$, $20\%$, $100\%$ & 4     & 0.9, 0.99, 0.999 \\
\DenseNetshort~\cite{huang2017densely} & CIFAR100 & LS, DML, SL, KD, CN \\% & $5\%$, $10\%$, $20\%$, $100\%$ & 4     & 0.9, 0.99, 0.999\\
\bottomrule
\end{tabular}
\end{center}
\end{table*}
%We considered $8$ different deep learning models. Due to infrastructure limitations, we focused on ResNet architectures (\ResnetS, \ResnetB, \DensenetS, \DensenetB, \ResnextS, \ResnextB, \SeResNext) and as a reference  \inceptionresnet. Since these models require moderate computational requirements they are used in practice extensively. ResNet class architectures belong to the most prominent and popular architectures for image classification, object detection and semantic segmentation  problems \cite{ren2015faster,dai2016r,he2017mask, chen2018deeplab}. 
For all architectures, we have followed the experimental protocols described in the original publications \cite{he2016deep,zagoruyko2016wide,xie2017aggregated,hu2018squeeze,szegedy2017inception,huang2017densely}. % as  supplied in the Appendix for completeness.
All experiments were conducted using the PyTorch deep learning library \cite{paszke2017automatic}.\footnote{The code to reproduce our results is available in the supplementary material.} For all experiments, except ImageNet $\DR=100\%$, we  used stochastic gradient descent (SGD) for optimization. For ImageNet $\DR=100\%$  we used the distributed SGD algorithm \cite{goyal2017accurate} with Horovod\footnote{Horovod is a method which uses large batches over multiple GPU nodes and some accuracy loss is expected  for the baseline method and this is well established. For more details please see Table~$1$ and Table $2$.c in  \cite{paszke2017automatic}.} \cite{sergeev2018horovod} support because of the computational demands.
%in order to scale the experimental design. 
The distributed SGD algorithm \cite{goyal2017accurate} is one of the state-of-the-art methods for large scale training. It is expected to lead to a slight loss in performance when a large batch size is used (see \cite{goyal2017accurate} for details). 

Our approach introduces the hyperparameter $\epsilon$, see \eqref{eq:eps}. %One can use standard model selection methods e.g. $k$-fold cross-validation or Bayesian optimization. However,
In order to assess the stability of the proposed method, we present results for $\epsilon \in \{0.9,0.99,0.999\}$.\footnote{We have tried $\epsilon \in \{0.8, 0.9, 0.91, \ldots,$ $0.98, 0.99, 0.992, \ldots,$ $0.998, 0.999\}$ for \ResnetS\ and \ResnetB. The results showed that the search space for $\epsilon$ can be less granular and we have limited the search space accordingly.} We repeated all experiments four times. We report the top-$1$ and top-$5$ classification accuracy on the \ask{test} datasets (standard deviations are  reported in the supplementary material). 

%For calculating the label similarity, we tested different \texttt{doc2vec} embedding dimensions $d\in\{50, 100, 150, 200, 250, 300\}$ with \ResnetS\ and \ResnetB. We did not observe any significant differences in the classification accuracies. Hence, we only report results for  the $d=100$ dimensional \texttt{doc2vec} embeddings.

For estimating the label similarity matrix, we  used \emph{pretrained} \texttt{doc2vec} emebeddings with dimensions $d\in\{100, 300, 500\}$ with \ResnetS\ and \ResnetB. We did not observe any significant differences in the classification accuracies. The maximum difference between compatible settings were less than 0.06 \%. Hence, we only report results for  the $d=100$ dimensional \texttt{doc2vec} embeddings.

For each experiment, we used workstations having 4 Tesla P100 GPUs (with 16GB GPU RAM) each. For network communication we used InfiniBand, which is a computer-networking communications standard designed for high throughput and low-latency scenarios. %If all experiments would have been conducted in parallel, approximately 9.2K Tesla P100 GPUs would have been required.


%We did not tune any of the original hyperparameters (e.g., learning rates) of the models for our method. But note that these hyperparameters were tuned for the baseline. 
We tuned the hyperparameters for the baseline method (SL) only. For 100\% data, we took the hyperparameters from the original publications. For all other settings, we optimized learning rate, batch size and weight-decay for the standard baseline (SL). Then we use the very same parameters for our approach (we just varied the new parameter epsilon). Thus, hyperparameter tuning would rather increase the gain from using our method.
Thus, one might argue that the new algorithm is using sub-optimal hyperparameters compared to the baselines. However, our goal was to  show that the proposed algorithm can improve any model on different datasets without tuning hyperparameters.




==> mgqvjdvbgzvywcqgtdzyrbkbyvpwvyqs/implementation.tex <==
We have evaluated our curriculum  learning strategy on $8$ different models. Due to infrastructure limitations, we have focused on Resnet class architectures (Resnet-$50$, Resnet-$152$, Densenet-$121$, Densenet-$161$, Resnext-$101-32\times{}4d$, Resnext-$101-64\times{}4d$ ,SeResNext-$101-32\times{}4d$) and for completeness InceptionResnetv2. Since these models require moderate computational requirements they are used in practice extensively. Resnet class architectures belong to the most prominent and popular architectures for image classfication, object detection and semantic segmentation  problems \cite{ren2015faster,dai2016r,he2017mask, chen2018deeplab}. 

For all architectures for data processing and data augmentation, we have followed the experimental protocol which is described in the corresponding original publication. All experiments are conducted by using PyTorch deep learning libray\cite{paszke2017automatic}. We conduct a large scale experimantal study, therefor we have used distributed SGD algorithm \cite{goyal2017accurate} with Horovod \cite{sergeev2018horovod} support in order to scale the experimental design. The used distributed SGD algorithm \cite{goyal2017accurate} is one of the state-of-the-art methods for large scale training. It is expected to observe slight loss of performance whenever large batch size is used (please see the results presented in \cite{goyal2017accurate}). For classical ResNet architectures and DenseNet architectures, we recover the accuracy loss. For some of the  models, we are not able recover the accuracy loss compared the published baseline. However, we improve over reproduced results by using large batch solver.



%Optimisation is performed using synchronous SGD with momentum 0.9 and a mini-batch size of 1024. The initial learning rate is set to 0.6 and decreased by a factor of 10 every 30 epochs. All models are trained for 100 epochs from scratch, using the weight initialisation strategy described in [9]. 


  

==> mgqvjdvbgzvywcqgtdzyrbkbyvpwvyqs/related_work.tex <==
Starting from the work by  Bengio et  al.~\cite{bengio2009curriculum}, a variety of curriculum learning  approaches has been
studied. However, they all define a curriculum at the level of
training examples. For instance, \emph{self-paced learning} by 
Kumar et al.~\cite{kumar2010self}
%assume
%        that easy examples are the examples for which the output can
%        be predicted easily. They introduce
%
%self-paced learning
introduces 
latent variables for modelling ``easiness'' of an examples.
% and solve a (relaxed) mixed integer program.
Graves et al.~\cite{graves2017automated} consider example-based
improvement measures as reward signals for multi-armed bandits, which
then build stochastic syllabi for neural networks.
%They consider range of signals that determine improvement like rate of increase in prediction accuracy and rate of increase in network complexity 
\review{
Florensa et al.~\cite{florensa2017reverse} study curriculum learning
in the context of reinforcement learning in robotics. They propose to
train a robot by gradually increasing the complexity of the task at
hand (e.g., the  robot learns to reach a goal by setting starting points increasingly far from the goal).} 
\review{
In recent work, Weinshall et al.~\cite{weinshall2018curriculum}
%propose two methods for curriculum learning. In the first one, they
consider learning tasks with convex linear regression loss and prove
that the convergence rate of a
perfect curriculum learning method increases with the difficulty of the examples. In addition, they propose a  method which infers the curriculum
using transfer learning from another network (e.g., \ResnetS)
pretrained on a different task. They train a linear classifier using
features extracted from the pretrained model and score each training
example using the linear classifier’s confidence (e.g., the
margin of an SVM).
% and consider the confidence score as curriculum scores.
Finally, they train a smaller deep neural network for the transfer
learning task following a curriculum based on these scores.} 

Buciluǎ et al.~\cite{bucilua2006model} have  proposed compressing a large model into a simple model which  reduces space requirements and increases inference speed at the cost of a small performance loss. This idea has been revisited in  \cite{hinton2015distilling} under the name  \emph{knowledge distillation} (KD) and received a significant amount of attention (e.g., \cite{papernot2016distillation,romero2014fitnets,zagoruyko2016paying,yim2017gift,orbes-ortega:19b}).
KD  methods typically require a pretrained model to start with or train a series of models on the same training data.
%\footnote{A complete list of all references is beyond scope of this paper. Hence, we have only mentioned a set of representative papers.}
Standard KD considers a teacher network and a student network. 
The 
%flexible With the help of a 
powerful teacher network is used to support the  training  of the student network which may be less complex or may have access to less data for training. KD is related to curriculum learning methods because the teacher network guides the learning of student networks \cite{hinton2015distilling}. A variant of KD,  \emph{born again neural network}, trains a series of models, not only one \cite{furlanello2018born}. 
%As far as authors are aware of, most if not all, 



\emph{Deep mutual learning} (DML) is also loosely related to our proposed approach \cite{hinton2015distilling,zhang2018deep}.  In DML, two models  solve the same classification problem collaboratively and are jointly optimised   \cite{zhang2018deep}. Each model acts as a teacher for the other model, and each network is trained with two losses. The first loss is the standard cross-entropy  between the model's predictions and target labels. The second  is a \emph{mimicry loss} that aligns both model's class posteriors with the class probabilities of the respective other  model. 
%

Another related approach is \emph{CurriculumNet} \cite{guo2018curriculumnet}, a clustering based curriculum strategy for learning from noisy data. CurriculumNet consists of three steps. First, a deep neural network is trained on the noisy label data. Second, features are extracted by using the model trained in the first step. Using clustering algorithms, these features are then grouped into different sets and sorted into easy and difficult examples. Finally, a new deep neural network is trained using example-weighted curriculum learning. Sorting of examples from easy to hard and clustering algorithms add many hyper-parameters (e.g., number of clusters), and one has to train two neural network models of almost the same size.
%Points near to cluster centers are considered as easy examples and points away from cluster centers are considered as hard examples

Our algorithm can be considered as a multi-modal deep learning method,  where text data is used for estimating the class similarity matrix to improve image classification. 
%Note that text data is not always needed if one can build label similarity using other information. 
However, it is different from standard multimodal methods as it does not use text data as an input to the deep neural network. The \emph{DeVise} algorithm is a popular multi-modal method which utilizes the text modality in order to learn a mapping from an image classifier's feature space to a semantic space.   \cite{frome2013devise}. {DeVise} requires a pretrained deep neural network. Furthermore, as  stated in \cite{frome2013devise}, it does not improve the accuracy on the original task but  aims at training a  model for zero-shot learning.
%Furthermore, our algorithm is also different from \emph{DeVise} .  

There is an obvious relation between LCL and \emph{label smoothing} (LS) \cite{muller2019does}, which we will discuss in Section~\ref{sec:experiments}. 

The computational requirements of KD, DML,  and CurriculumNet  are significantly higher compared to our method, which is rather simple. Furthermore, our method does not require training more than one model and adds only a single  hyper-parameter. 
%Furthermore, as far as we are aware of, most curriculum learning methods train on the target training data, while our method can utilize an additional modality efficiently.



==> mgqvjdvbgzvywcqgtdzyrbkbyvpwvyqs/results.tex <==
\begin{figure}[t!]
	\includegraphics[width=.32\linewidth]{figures/Eigenvalues_ImageNet.png}
	\includegraphics[width=.32\linewidth]{figures/Eigenvalues_Cifar100.png}
	\includegraphics[width=.32\linewidth]{figures/Eigenvalues_AwA2.png}
	\caption{Eigenvalue distributions of the class similarity matrices for ImageNet, \cifar{}, and AwA2.}
	\label{fig:eig_imagenet_class_dis_matrix}
\end{figure}

We will focus on the results for ImageNet, CIFAR100, and AWA2 and the similarity measure introduced in Section~\ref{sec:proposed_method},  result tables for the other data sets and other similarity measures can be found in
the supplementary material.
%sections  \ref{app:awa}, \ref{app:nabirds}, and \ref{app:cub}.
Before we present the learning results, we will discuss the structure of the label similarity matrices for the data sets ImageNet, CIFAR100, and AWA2.

%\subsection{Label Similarities}
\paragraph{Label Similarities.}
%\ci{I like the eigenspectrum analysis. But it should not be in the conclusions. Actually, I think it should be in the beginning of the Results \& Discussion section.}
For a better understanding of the label similarity matrices, we visualized their eigenspectra in Figure~\ref{fig:eig_imagenet_class_dis_matrix}. %--\ref{fig:eig_awa2_class_dis_matrix}.
Consider two extreme scenarios:
%rank-1 label similarity matrix and rank-n label similarity matrix with equal eigenvalues. In the rank-1 case, 
If a label similarity matrix has rank 1, all classes are exactly the same and there cannot be any discriminatory learning. In contrast,  the full rank case with equal eigenvalues is the standard learning case where all classes are orthogonal  to each other (one-hot-encoding). 
%But reality lies in between: in 
Figure~\ref{fig:eig_imagenet_class_dis_matrix}
%, we plot eigenvalues of a label similarity matrix for ImageNet. Note that there is 
shows  exponential eigenvalues decays, which means there are clusters of similar classes. Distinguishing between these clusters of classes is an easier task than distinguishing between classes within one cluster. 
%Such eigenvalue decay, allows for both discriminative learning between classes and curriculum learning. 





\begin{table}[ht!]
{%\tiny
    \begin{center}
{
\caption{ImageNet. Top-1 results, averaged over four trials.}
\label{Tab:top_1_ImageNet}
\begin{tabular}{lccccccc}
{} & {} & {} & {} & {} &\multicolumn{3}{c}{$\boldsymbol{\epsilon}$}\\
\cmidrule{6-8}
{} & \textbf{SL} &             \textbf{LS} & \textbf{KD} & \textbf{CN} &          $\boldsymbol{0.9}$ &           $\boldsymbol{0.99}$ &     $\boldsymbol{0.999}$ \\
\midrule
&\multicolumn{7}{c}{DR = 5\%}\\
\cmidrule{2-8}
\ResnetS          &    38.21 &   38.43 & 39.81 & 36.12 & 41.24 &    41.6 &  \textbf{42.21} \\
\ResnextSshort &   45.46 &   45.71 &  46.21 & 44.14 &  46.1 &   46.92 &  \textbf{47.12} \\
\SENet         &   48.29 &   48.57 &   48.44 & 46.21 & 49.8 &   50.04 & \textbf{50.19} \\
\cmidrule{2-8}
&\multicolumn{7}{c}{DR = 10\%}\\
\cmidrule{2-8}
\ResnetS          &   51.95 &   52.25 &  53.64 & 52.17 & 55.39 &   55.62 &  \textbf{55.64} \\
\ResnextSshort &   58.63 &   58.92 &   58.94 & 57.64 & 59.78 &   \textbf{60.07} &  59.92 \\
\SENet        &   60.61 &   60.74 & 60.82 & 60.14 & 60.99 &   61.18 &  \textbf{62.28} \\
\cmidrule{2-8}
&\multicolumn{7}{c}{DR = 20\%}\\
\cmidrule{2-8}
\ResnetS          &   61.87 &    62.11 &   63.17 & 62.41 & 64.41 &   64.42 &   \textbf{64.44} \\
\ResnextSshort &   67.96 &   68.13 & 68.29 & 68.14 &  68.48 &   68.47 &  \textbf{68.57} \\
\SENet         &   67.77 &   67.71 & 67.64 & 67.43 &  68.14 &   \textbf{68.4} &  68.33 \\
\cmidrule{2-8}
&\multicolumn{7}{c}{DR = 100\%}\\
\cmidrule{2-8}
\ResnetS          &   76.25 &    76.4 & 76.38 & 76.1 & 76.71 &   76.75 &  \textbf{76.89} \\
\ResnextSshort &   78.05 &  78.17  & 78.21 & 77.94 & 78.31 &    78.5 &  \textbf{78.64} \\
\SENet         &   79.33 &   79.65 &   79.44 & 79.44 & 80.11 &   80.03 &  \textbf{80.21} \\
\bottomrule
\end{tabular}
}
\end{center}
}
\end{table}

\begin{table}[ht!]
\begin{center}
\caption{ImageNet. Top-5 results, averaged over four trials.}
\label{Tab:top_5_ImageNet}
\begin{tabular}{lccccccc}
{} & {} & {} & {} & {} &\multicolumn{3}{c}{$\boldsymbol{\epsilon}$}\\
\cmidrule{6-8}
{} & \textbf{SL} &             \textbf{LS} &    \textbf{KD} & \textbf{CN} &        $\boldsymbol{0.9}$ &           $\boldsymbol{0.99}$ &     $\boldsymbol{0.999}$ \\
\midrule
&\multicolumn{7}{c}{DR = 5\%}\\
\cmidrule{2-8}
\ResnetS          &  64.04& 64.35& 67.22& 65.12
 & 64.41 & 67.59&  \textbf{67.94}\\
\ResnextSshort           &  70.52& 70.76& 71.84& 70.92 & 70.67 & 72.05&  \textbf{72.18}\\
\SENet            &  73.35& 73.52& 74.54& 73.92
 & 73.56 & 74.65&  \textbf{74.92}\\
\cmidrule{2-8}
&\multicolumn{7}{c}{DR = 10\%}\\
\cmidrule{2-8}
\ResnetS          &  76.86&  77.04& 79.73& 78.14 & 77.1 & \textbf{79.8}&   79.69\\
\ResnextSshort           &  81.52&  81.87& 82.56& 81.92 &	81.67 & 82.66&  \textbf{82.74}\\
\SENet             &  82.53&  \textbf{83.71}& 83.38& 82.76 &	82.94 & 83.6&   83.5\\
\cmidrule{2-8}
&\multicolumn{7}{c}{DR = 20\%}\\
\cmidrule{2-8}
\ResnetS          &  84.41&  84.57& 86.1& 85.36 &	84.91 &  \textbf{86.15}&  86.14\\
\ResnextSshort           &  87.96&  88.11& 88.2& 88.04	& 87.84 & \textbf{88.36}&  \textbf{88.36}\\
\SENet            &  88.16&  88.23& 88.17& 88.17 &	88.11 & \textbf{88.37}&  88.31\\
\cmidrule{2-8}
&\multicolumn{7}{c}{DR = 100\%}\\
\cmidrule{2-8}
\ResnetS          &  92.87&  92.91& 92.94& 92.41 &	92.84 & \textbf{92.95}&  92.93\\
\ResnextSshort           &  93.95&  93.92& 93.96& 93.85 &	93.87 & 94.07&  \textbf{96.15}\\
\SENet            &  94.33&  94.44& 94.84& 94.02 &	94.35 & \textbf{94.93}&  94.79\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

\begin{table}[ht]
    \begin{center}
\caption{\cifar{}. Top-1 results, averaged over four trials.}
\label{Tab:top_1_CIFAR100}
\begin{tabular}{lccccccccc}
{} & {} & {}& {} &{}& {} &{} &\multicolumn{3}{c}{$\boldsymbol{\epsilon}$}\\
\cmidrule{8-10}
{} & \textbf{SL} &            \textbf{LS} &      \textbf{DML}$_{\boldsymbol{1}}$ &  \textbf{DML}$_{\boldsymbol{2}}$ &   \textbf{KD} & \textbf{CN} &          $\boldsymbol{0.9}$ &           $\boldsymbol{0.99}$ &     $\boldsymbol{0.999}$\\
\midrule
&\multicolumn{9}{c}{DR = 5\%}\\
\cmidrule{2-10}
\WRNshort              &    40.2 &  40.31 &  40.16 & 40.47 & 40.94 & 38.14 & 41.36&  41.86 & \textbf{41.92} \\
\DenseNetshort    & 43.34 & 43.5 &  43.89 & 44.14 & 43.76 & 43.42 &  \textbf{44.66}& 45.37&  44.53\\
\cmidrule{2-10}
&\multicolumn{9}{c}{DR = 10\%}\\
\cmidrule{2-10}
\WRNshort               & 60.2 &   60.1 &  60.38 &  60.34 & 60.45 & 60.14  &  60.49 &  60.86&  \textbf{61.19} \\
\DenseNetshort &   60.85&   61.1 &  61.22 &  61.34 & 60.81 & 59.83  &   61.5 & 61.4&  \textbf{61.65} \\
\cmidrule{2-10}
&\multicolumn{9}{c}{DR = 20\%}\\
\cmidrule{2-10}
\WRNshort               &   71.05 &  71.25& 71.61 &  71.65 & 71.53 & 71.37  &  71.64& 71.67 &  \textbf{
71.83} \\
\DenseNetshort &   72.38 & 72.39 &   71.5&  71.34 & 72.24 & 71.54 &  72.71&  72.65 &  \textbf{72.87} \\
\cmidrule{2-10}
&\multicolumn{9}{c}{DR = 100\%}\\
\cmidrule{2-10}
\WRNshort               &   79.52 &  79.84 & 80.32&  80.20 & 80.14 & 78.64    &  81.17 &  81.15 &  \textbf{81.25} \\
\DenseNetshort &   82.85 &  83.01 &  82.91 &  82.57 & 82.67 & 81.14 &  82.96 &  83.11 &   \textbf{83.2} \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

\begin{table}[ht!]
    \begin{center}
    \caption{\cifar{}. Top-5 results, averaged over four trials.}
\label{Tab:top_5_CIFAR100}
    {\begin{tabular}{lccccccccc}
{} & {} & {}& {} &{} & {} &{} &\multicolumn{3}{c}{$\boldsymbol{\epsilon}$}\\
\cmidrule{8-10}
{} & \textbf{SL} &            \textbf{LS} &    \textbf{DML}$_{\boldsymbol{1}}$ &  \textbf{DML}$_{\boldsymbol{2}}$ &     \textbf{KD} & \textbf{CN} &         $\boldsymbol{0.9}$ &           $\boldsymbol{0.99}$ &     $\boldsymbol{0.999}$\\
\midrule
&\multicolumn{9}{c}{DR = 5\%}\\
\cmidrule{2-10}
\WRNshort               &   68.82  &  68.95  &  68.74  &  68.89  & 68.94 &	69.12 &   69.47&  69.39  &  \textbf{69.63}  \\
\DenseNetshort          &   70.61  &  70.85  &   70.7  &  70.92  & 71.14 &	71.27 &   72.1 &  71.13  &  \textbf{72.52}  \\
\cmidrule{2-10}
&\multicolumn{9}{c}{DR = 10\%}\\
\cmidrule{2-10}
\WRNshort               &   83.64  &  83.82  &  84.05  &  84.11 & 83.94 &	83.77 &  83.99 &  84.15  &   \textbf{84.3}  \\
\DenseNetshort          &   84.07  &  84.21  &  84.27  &  84.45 & 84.07 & 84.31 &  84.34 &  \textbf{84.63}  &  84.52  \\
\cmidrule{2-10}
&\multicolumn{9}{c}{DR = 20\%}\\
\cmidrule{2-10}
\WRNshort               &   90.52  &  90.38  &   90.3  &  90.27  & 90.71 & 90.45 &  91.02 &  \textbf{91.19}  &   90.95 \\
\DenseNetshort         &   91.24  &  91.37  &  91.33  &  91.30  & 91.39 & 91.38 &   91.4 &  91.31  &  \textbf{91.47}  \\
\cmidrule{2-10}
&\multicolumn{9}{c}{DR = 100\%}\\
\cmidrule{2-10}
\WRNshort              &   94.04  &  94.23  &  94.44  &  94.42  & 94.52 &	94.52 &   95.29&  95.17  &  \textbf{95.49}  \\
\DenseNetshort          &   95.22  &  95.28  &  95.34  &  95.27  & 95.37 &	95.63 &  95.72 &   95.74 &  \textbf{95.88}  \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}


\begin{table}[ht!]
    \begin{center}{\caption{AWA2. Top-1 results, averaged over four trials.}
\label{Tab:top_1_AWA2}
\begin{tabular}{lccccccccc}
{} & {} & {}& {} &{} & {} &{} &\multicolumn{3}{c}{$\boldsymbol{\epsilon}$}\\
\cmidrule{8-10}
{} & \textbf{SL} &            \textbf{LS} &       \textbf{DML}$_{\boldsymbol{1}}$ &  \textbf{DML}$_{\boldsymbol{2}}$ &  \textbf{KD} & \textbf{CN} &             $\boldsymbol{0.9}$ &           $\boldsymbol{0.99}$ &     $\boldsymbol{0.999}$\\
\midrule
&\multicolumn{9}{c}{DR = 5\%}\\
\cmidrule{2-10}
\ResnetB         &   23.09  &  27.82 &  39.22 &  37.19 & 41.58       & 24.1  &  45.51 &  45.55  &  \textbf{45.78}   \\
\inceptionresnet &   57.42 &  57.95  &  58.69 &  58.14 & 59.3        & 56.9 &  60.85 &  \textbf{61.07}  &    60.71 \\
\cmidrule{2-10}
&\multicolumn{9}{c}{DR = 10\%}\\
\cmidrule{2-10}
\ResnetB         &   41.86 &  44.98  &  48.92 &   50.5& 44.02       & 43.12 &  47.21 &  51.67  &   \textbf{53.39}  \\
\inceptionresnet &    71.47&  71.86  &  71.82 &  72.37 & 71.49       & 72.01 &  72.61 &  72.97  &   \textbf{73.01}  \\
\cmidrule{2-10}
&\multicolumn{9}{c}{DR = 20\%}\\
\cmidrule{2-10}
\ResnetB         &   77.11 &  78.23  &   78.34&  78.32 & 78.28       & 77.64 &  80.03 &  \textbf{80.07}  &   79.86  \\
\inceptionresnet &   83.64 &  83.92  &  83.87 &  83.76 & 83.83       & 84.12 &  \textbf{84.27} &  84.05  &   \textbf{84.27}  \\
\cmidrule{2-10}
&\multicolumn{9}{c}{DR = 100\%}\\
\cmidrule{2-10}
\ResnetB         &   88.73 &  89.25  &  89.01 &  89.11  & 89.17       & 88.92  &  89.44 &  \textbf{89.64}  &   89.63  \\
\inceptionresnet &   89.69 &  89.94  &  90.05 &  90.22 & 89.94       & 89.29 &  \textbf{90.49} &  90.34  &   90.47  \\
\bottomrule
\end{tabular}
}
\end{center}

\end{table}


\begin{table}[ht!]
    \begin{center}{\caption{AWA2. Top-5 results, averaged over four trials.}
\label{Tab:top_5_AWA2}
\begin{tabular}{lccccccccc}
{} & {} & {}& {} &{}& {} &{} &\multicolumn{3}{c}{$\boldsymbol{\epsilon}$}\\
\cmidrule{8-10}
{} & \textbf{SL} &            \textbf{LS} &    \textbf{DML}$_{\boldsymbol{1}}$ &  \textbf{DML}$_{\boldsymbol{2}}$ &  \textbf{KD} & \textbf{CN} &             $\boldsymbol{0.9}$ &      $\boldsymbol{0.99}$ &         $\boldsymbol{0.999}$ \\
\midrule
&\multicolumn{9}{c}{DR = 5\%}\\
\cmidrule{2-10}
\ResnetB         &   53.31  &  54.19 &  65.14 &    63.12 &  56.19 & 54.17  &76.02  &  76.14  &  \textbf{76.47}  \\
\inceptionresnet &   83.06  &  83.14  &  84.07  &  84.18 & 84.12 &	83.77 & 84.94  &  \textbf{85.24}  &  84.84  \\
\cmidrule{2-10}
&\multicolumn{9}{c}{DR = 10\%}\\
\cmidrule{2-10}
\ResnetB         &   72.59  &  72.43  &  75.07  &  76.14 & 76.61 &	76.34 & 77.04  &  \textbf{80.46}  &  80.11  \\
\inceptionresnet &   91.37  &  91.42  &  91.35  &  91.43 & 91.48	& 91.35 &  \textbf{91.9}  &  91.89  &   91.71 \\
\cmidrule{2-10}
&\multicolumn{9}{c}{DR = 20\%}\\
\cmidrule{2-10}
\ResnetB         &   94.21  &  94.56  &  94.79  &  95.01 &  94.61	& 94.45 & \textbf{95.2}  &  95.07  &  95.12  \\
\inceptionresnet &   96.03  &  96.23  &  96.28  &  96.13 &  96.21 &	95.19 &96.18  &  96.49  &  \textbf{96.57}  \\
\cmidrule{2-10}
&\multicolumn{9}{c}{DR = 100\%}\\
\cmidrule{2-10}
\ResnetB         &   97.85  &  97.92  &   98.1  &  97.95 & 97.43 &	97.32 & 98.11  &  \textbf{98.14}  &   98.1  \\
\inceptionresnet &   98.01  &  98.07  &  98.25  &   98.17& 97.67 &	97.56 & 98.25  &  \textbf{98.41}  &   98.2  \\
\bottomrule
\end{tabular}
}
\end{center}

\end{table}



%\subsection{Classification Performance}
\paragraph{Classification Performance.}
We measured the  top-$1$ classification accuracy and top-$5$ classification
accuracy after the last epoch. The results are summarized in Table \ref{Tab:top_1_ImageNet} and Table \ref{Tab:top_5_ImageNet} for ImageNet, in Table \ref{Tab:top_1_CIFAR100} and Table \ref{Tab:top_5_CIFAR100} for \cifar, and in Table \ref{Tab:top_1_AWA2} and Table \ref{Tab:top_5_AWA2} for AWA2 (for standard deviations see the supplementary material). All results are averaged over four trials.
%
It is important to keep in mind that we compare against baseline
results achieved with architectures and hyperparameters tuned for
excellent performance. %{Thus, there is little room for improvement.}
%
Furthermore, we compare to baseline results from our own experiments,
not to results taken from the literature. We ran each experiment 4 times with same seeds for all algorithms. This allows for a fair comparison. Our averaged results also provide a more reliable estimate of the performance of the systems compared to single trials reported in the original works.

% show that
% the proposed method outperformed the corresponding \emph{reproduced}
% baseline for all cases except one case per each metric.

%When looking at the top-1 results and the 7 architectures for which we
%tested larger values of $\epsilon$, we see that the baseline was always
%outperformed by curriculum learning with either
%$\epsilon = 0.85$ or $\epsilon = 0.95$. In particular,
%$\epsilon = 0.95$ performed best in 6 out of the 7 cases and better than the
%baseline in also 6 cases.


%For \inceptionresnet{}, we (so far) have only results for the baseline
%and $\epsilon = 0.2$ or $\epsilon = 0.3$. Both curriculum learning
%settings outperformed the baseline, $\epsilon = 0.2$ reaching an
%average accuracy of 80.457 after the final epoch. \footnote{The
%  experiments for \inceptionresnet\ were still running at the time of
%  submission. So far, we only have results for $\epsilon \in
%  \{0.2,0.3\}$, which already support our curriculum learning
%    approach. The missing results will be added before the rebuttal
%    period. Given the current results, it can be expected that the trials with higher $\epsilon$ values will %lead to even higher accuracies.  }

%There seems to be a tendency that the curriculum learning
%is particularly helpful for deep networks,  for example, compare  Resnet$152$ vs.{} Resnet$50$ and %Densenet$161$ vs.{}  Densenet$121$.

The results show that for all datasets and in  all experimental cases using {LCL} outperformed all baselines, with SeNet with $\DR=10\%$ and top-5 metric being the only exception. The improvement was more pronounced when $\DR < 100\%$. It is quite intuitive that a curriculum is much more important when the training data is limited (i.e., the learning problem is more difficult). Loosely speaking, the importance of a teacher decreases when a student has access to unlimited  information without any computational and/or time budget. 


For example, for \ResnetS on ImageNet  {LCL} improved the top-1 accuracy on average by $4$ percentage points (p.p.) over the baseline when $\DR = 5\%$, and  2\,p.p.\ in top-5 accuracy were gained with  $\DR = 100\%$ on ImageNet for the ResNeXt architecture.
%and improves by $2\%$ when  $\DR = 100\%$ on ImageNet dataset. 
The biggest improvements were achieved on the AWA2 dataset.
For \ResnetB and $\DR = 5\%$,  average improvements of  more than 22\,p.p.\ and 23\,p.p.\ could be achieved  in the top-1 and top-5 accuracy, respectively.
%
As could be expected, the performance gains in the top-$5$ setting were typically smaller than for top-$1$. Still, nothing changed with respect to the ranking of the network architectures. 

Larger values of $\epsilon$ mean slower convergence to the
one-hot-encoding and therefore more emphasis on the curriculum
learning. In most experiments, 
%$75\%$ of the time 
$\epsilon = 0.999$ performed best.
The observation that larger $\epsilon$ values gave better results than small ones
provides additional evidence that the curriculum really
supports the learning process (and that we are not discussing random artifacts).

Under the assumption that the experimental scenarios are statistically independent, we performed a 
{statistical comparisons of the classifiers over
multiple data sets for all pairwise comparisons} following \cite{demvsar2006scc,garcia2008esc}.
Using the Iman and Daveport test, all but one result were statistically significant. If we consider all  ImageNet top-1 accuracy results, our method with $\epsilon=0.999$  ranked best, followed by $\epsilon=0.99$, $\epsilon=0.9$, LS and then SL. This ranking was highly significant (Iman and Daveport test,  $p<0.001$). Similarly, our method with $\epsilon=0.999$ was best for both CIFAR-100 and AWA2 ($p<0.001$). 

%The only outlier was the \SeResNext\ architecture, where curriculum
%learning with  $\epsilon = 0.2$ gave the best results.
%The average top-5 accuracy
%achieved with the \inceptionresnet{}  architecture and
%$\epsilon = 0.2$ was 95.487.

%Figure~\ref{fig:evo} depicts the top-1 accuracies for \ResnetB,
%\DensenetB, \ResnextB, and \inceptionresnet\ for best performing cooling
%factors over the course of learning.  The plots show that -- given the
%hyperparameters optimized for the baselines -- the curriculum slows
%down the learning process in terms of accuracy to achieve consistently
%higher accuracies in the final epochs. The latter shows that the corresponding
%results in the tables are not dominated by random fluctuations in the
%last epochs of training.

%There could be several reasons for the slower learning. The first
%could be that the curriculum learning simply requires a higher
%learning rate.
%However, it  may also  be a natural consequence of the loss function.
%The loss function used in the curriculum learning is a worse surrogate
%for the classification accuracy  than the canonical cross-entropy, to
%which the curriculum loss converges. Thus, in the beginning reducing
%the loss and increasing the overall (not weighted) accuracy are less
%tightly coupled. 


%
%\begin{figure}
%	\includegraphics[width=\linewidth]{figures/overall_perf_top_1_intersect.png}
%	\caption{Top1 performance improvment/loss per model and cooling factor for proposed method compared to reproduced baseline}
%	\label{fig:top_1}
%\end{figure}


%\begin{figure}
%	\includegraphics[width=\linewidth]{figures/overall_perf_top_5_intersection.png}
%	\caption{Top5 performance improvment/loss per model and cooling factor for proposed method compared to reproduced baseline}
%	\label{fig:top_5}
%\end{figure}


%Because of limited space we only present detailed results for our best models in Figure \ref{fig:detailed_results}. Given the presented overall results in Figure \ref{fig:per_imp_overall} and detailed results, the proposed methods clearly outperforms the baselines.  
%\begin{figure*}
%	\begin{multicols}{2}
%		\includegraphics[width=\linewidth]{figures/\ResnetS_085.png}\par 
%		\includegraphics[width=\linewidth]{figures/resnet152_095.png}\par 
%	\end{multicols}
%	\begin{multicols}{2}
%		\includegraphics[width=\linewidth]{figures/densenet121_06.png}\par
%		\includegraphics[width=\linewidth]{figures/densenet161_095.png}\par
%	\end{multicols}
%	\begin{multicols}{2}
%		\includegraphics[width=\linewidth]{figures/resnext101_32x4d_06.png}\par 
%		\includegraphics[width=\linewidth]{figures/resnext101_64x4d_095.png}\par 
%	\end{multicols}
%	\begin{multicols}{2}
%		\includegraphics[width=\linewidth]{figures/se_resnext101_32x4d_02.png}\par 
%		\includegraphics[width=\linewidth]{figures/inceptionresnetv2_02.png}\par 
%	\end{multicols}
%	\label{fig:detailed_results}
%	\caption{caption here}
%\end{figure*}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}



%\begin{figure*}
%	\begin{multicols}{2}
%		\includegraphics[width=\linewidth]{figures/Resnet-152.png}\par 
%		\includegraphics[width=\linewidth]{figures/InceptionResNetV2.png}\par 
%	\end{multicols}
%	\begin{multicols}{2}
%		\includegraphics[width=\linewidth]{figures/DenseNet-161.png}\par 
%	\includegraphics[width=\linewidth]{figures/ResNeXt-101-64.png}\par
%	\end{multicols}
%	\caption{Top-1 accuracy results for \ResnetB, \DensenetB,
%          \ResnextB, and \inceptionresnet\ for the best performing cooling factors.\label{fig:evo}}
%\end{figure*}

